Discovery of Keys for Graphs [Extended Version]

Keys for graphs uses the topology and value constraints needed to uniquely identify entities in a graph database. They have been studied to support object identification, knowledge fusion, data deduplication, and social network reconciliation. In this paper, we present our algorithm to mine keys over graphs. Our algorithm discovers keys in a graph via frequent subgraph expansion. We present two properties that define a meaningful key, including minimality and support. Lastly, using real-world graphs, we experimentally verify the efficiency of our algorithm on real world graphs.

==> response.tex <==
\pagenumbering{gobble}

\begin{center}
%\textbf{Response Letter} \\
%\vspace{1em}
\textbf{Next Steps}
\end{center}
\label{sec-response}
%\vspace{1.8ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent{\bf Reviewer 1.}  
The author proposes an algorithm for mining keys from graphs, the first algorithm dedicated to keys apart from a preliminary workshop paper by the author. The definition of keys is that from Fan et al. Apart from the algorithm, the author has conducted an experimental study on two real-world graphs, providing some insight into the runtime performance of the algorithm based on some variations in the choice of parameters.

On the positive side, the paper addresses an important and technically challenging problem, is quite well motivated and presented, contributes an algorithm together with some optimisations, and conducts a reasonable performance evaluation.

On the negative side, there are a few questions that need to be addressed before acceptance can be warranted:
\begin{enumerate}
    
    \item It is stated that the keys studied in this paper form a special case of graph functional dependencies for which a mining algorithm exists: Wenfei Fan, Chunming Hu, Xueli Liu, Ping Lu: Discovering Graph Functional Dependencies. ACM Trans. Database Syst. 45(3): 15:1-15:42 (2020)

    It is further stated that the mining algorithm does not apply to keys. The argument presented why this is not applicable is not clear at all, so this needs clarification.
    \blue{I have clarified it further on why GFD discovery algorithm cannot mine keys.}
    
    \item There is a plethora of work on mining keys from data in other data models, some of which are cited by the author. These include approximate keys where the measures of support and minimality have been applied. The related work section should really emphasise how the methods of the author extend previously used methods. Based on the given body of techniques, it is necessary to see a clear line of extensions to accommodate new features of more powerful data model.
    
    \begin{enumerate}
    
        \item Renzo Angles, Angela Bonifati, Stefania Dumbrava, George Fletcher, Keith W. Hare, Jan Hidders, Victor E. Lee, Bei Li, Leonid Libkin, Wim Martens, Filip Murlak, Josh Perryman, Ognjen Savkovic, Michael Schmidt, Juan F. Sequeda, Slawek Staworko, Dominik Tomaszuk: PG-Keys: Keys for Property Graphs. SIGMOD Conference 2021: 2423-2436
    
        \item Johann Birnick, Thomas Bläsius, Tobias Friedrich, Felix Naumann, Thorsten Papenbrock, Martin Schirneck: Hitting Set Enumeration with Partial Information for Unique Column Combination Discovery. Proc. VLDB Endow. 13(11): 2270-2283 (2020)
        
        \item Eduardo H. M. Pena, Eduardo C. de Almeida, Felix Naumann: Discovery of Approximate (and Exact) Denial Constraints. Proc. VLDB Endow. 13(3): 266-278 (2019)
        
        \item Ziheng Wei, Uwe Leck, Sebastian Link: Discovery and Ranking of Embedded Uniqueness Constraints. Proc. VLDB Endow. 12(13): 2339-2352 (2019)
        
        \item Philipp Skavantzos, Kaiqi Zhao, Sebastian Link: Uniqueness Constraints on Property Graphs. CAiSE 2021: 280-295
        
        \item Sebastian Link: Neo4j Keys. ER 2020: 19-33
        
        \item Henning Köhler, Uwe Leck, Sebastian Link, Xiaofang Zhou: Possible and certain keys for SQL. VLDB J. 25(4): 571-596 (2016)
        
        \item Marcelo Arenas, Jonny Daenen, Frank Neven, Martín Ugarte, Jan Van den Bussche, Stijn Vansummeren: Discovering XSD Keys from XML Data. ACM Trans. Database Syst. 39(4): 28:1-28:49 (2014)

    \end{enumerate}

    \blue{I will cover these papers for the related work of the thesis, but I am not sure if we have space to cover it for the camera ready. For the full version to be uploaded to arXiv, I will use the most recent related work.}

    \item The experimental evaluation covers mostly performance issues. It should clearly state how many keys have been discovered, as the runtime is typically influenced by that. There is also some kind of qualitative evaluation missing. For at least some of the keys that have been discovered it should show what these keys are and how they are useful, eg. in terms of some of the application areas indicated.
    
    \blue{The qualitative experiments are added in the thesis draft. I will add it to the full version of this draft as well. But, do we have space to add it to the CR version?}
\end{enumerate}

My recommendation is to address these shortcomings in favour of some technical details that can be put in a technical report that can be referenced and later on added in a journal extension.

I propose to accept the paper conditionally on addressing the points (1-3) using a shepherd. If that cannot be done, I propose to reject the paper.

\vspace{1.8ex} \hrule \vspace{0.6ex} 

\noindent{\bf Reviewer 2.}  
In this paper, the author has proposed a technique for mining keys over directed labeled graphs. For experimentation, the author has been DBPedia and IMDb data sets. The paper has been well-written with examples, wherever necessary.

This paper can be made stronger if the following points are addressed

\begin{enumerate}

    \item The work has a close relation to existing work on frequent subgraph mining and graph querying. A short discussion comparing the two approaches may be beneficial.
    
    \item How does the author plan to handle the scenario of undirected graphs?
    
    \item The experiments and corresponding performance graphs have spoken about efficiency/run-time. However, there is no mention of accuracy comparison against the ground-truth mentioned in [20]. 
    \blue{Similar to R1.\#3. The experiment is added to the thesis draft and will be added to the full draft of this paper. But, do we have space to add it to the CR version?}
    
    \item There is some discrepancy in the results on page 11. At one point, it is mentioned 30\% faster, whereas at some point it is mentioned 28\% faster. Please provide results accurately. \blue{done.}
    
    \item Major comparisons have been shown for GKMiner and GKMiner-OPT. Is there no other algorithm, the proposed algorithm can be compared against. \blue{To be discussed.}
    
    \item The IMDb data set in [1] is present in a relational format. How were graphs created for experimentation? \blue{To be discussed.} Also please check the URL provided in the references. \blue{The URL works, but it is FTP and needs to be open by an appropriate app, like FileZilla.}

\end{enumerate}

\vspace{1.8ex} \hrule \vspace{0.6ex} 

\noindent{\bf Reviewer 3.} No specific comment

\vspace{1.8ex} \hrule \vspace{0.6ex} 

\noindent{\bf Reviewer 4.} No specific comment

\vspace{1.8ex} \hrule \vspace{0.6ex} 

